One Instrument to Rule Them All: The Bias and Coverage of Just-ID IV

We revisit the finite-sample behavior of single-variable just-identified instrumental variables (just-ID IV) estimators, arguing that in most microeconometric applications, the usual inference strategies are likely reliable. Three widely-cited applications are used to explain why this is so. We then consider pretesting strategies of the form $t_{1}>c$, where $t_{1}$ is the first-stage $t$-statistic, and the first-stage sign is given. Although pervasive in empirical practice, pretesting on the first-stage $F$-statistic exacerbates bias and distorts inference. We show, however, that median bias is both minimized and roughly halved by setting $c=0$, that is by screening on the sign of the \textit{estimated} first stage. This bias reduction is a free lunch: conventional confidence interval coverage is unchanged by screening on the estimated first-stage sign. To the extent that IV analysts sign-screen already, these results strengthen the case for a sanguine view of the finite-sample behavior of just-ID IV.

==> table1.tex <==
\multicolumn{9}{@{}c}{A. AK91}\\

 Men born 1920--29 & Log weekly wage & Years of education & Born in Q1 & 0.080 & -0.122 & -0.009 & 0.072& $0.043$ \\
  $(n=247,199)$ & [0.65] & [3.36] & [0.43] & (0.0004) & (0.016) & (0.003) & (0.023) & $(-0.210, 0.292)$  \\
 Men born 1930--39 &  &  &  & 0.071 & -0.106 & -0.011 & 0.105& $-0.175$ \\
  $(n=329,509)$ & [0.68] & [3.28] & [0.43] & (0.0004) & (0.013) & (0.003) & (0.025) & $(-0.407, 0.068)$  \\[1em]
\multicolumn{9}{@{}c}{B. AE98}\\
 1980 Census, mothers aged 18--35 & Worked for pay & More than 2 kids & Samesex & -0.176 & 0.061 & -0.007 & -0.117& $-0.058$ \\
  $(n=394,840)$ & [0.50] & [0.49] & [0.50] & (0.002) & (0.001) & (0.002) & (0.025) & $(-0.105, -0.010)$  \\
  & Weeks worked &  &  & -8.978 & 0.061 & -0.340 & -5.559& $-0.075$ \\
  & [22.29] & [0.49] & [0.50] & (0.071) & (0.001) & (0.069) & (1.118) & $(-0.122, -0.027)$  \\
 1990 Census, mothers aged 18--35 & Worked for pay &  &  & -0.164 & 0.062 & -0.006 & -0.092& $-0.069$ \\
  $(n=380,007)$ & [0.48] & [0.48] & [0.50] & (0.002) & (0.002) & (0.002) & (0.025) & $(-0.116, -0.022)$  \\
  & Weeks worked &  &  & -8.649 & 0.062 & -0.341 & -5.462& $-0.067$ \\
  & [22.87] & [0.48] & [0.50] & (0.077) & (0.002) & (0.073) & (1.156) & $(-0.114, -0.020)$  \\[1em]
\multicolumn{9}{@{}c}{C. AL99}\\

 5th grade, full sample & Reading & Class size & Maimonides' rule & 0.009 & 0.477 & -0.125 & -0.263& $0.357$ \\
  $(n=2,019)$ & [7.68] & [6.55] & [6.11] & (0.034) & (0.041) & (0.042) & (0.094) & $(0.207, 0.499)$  \\
  & Math &  &  & 0.036 & 0.477 & -0.126 & -0.264& $0.315$ \\
  & [9.60] & [6.54] & [6.10] & (0.045) & (0.041) & (0.056) & (0.123) & $(0.160, 0.462)$  \\
 5th grade, discontinuity sample & Reading &  &  & -0.070 & 0.481 & -0.197 & -0.410& $0.469$ \\
  $(n=471)$ & [8.18] & [7.42] & [7.50] & (0.050) & (0.057) & (0.050) & (0.118) & $(0.279, 0.639)$  \\
  & Math &  &  & 0.090 & 0.481 & -0.089 & -0.185& $0.322$ \\
  & [10.20] & [7.42] & [7.50] & (0.070) & (0.057) & (0.072) & (0.155) & $(0.107, 0.521)$  \\
